PaSe: An Extensible and Inspectable DSL for Micro-Animations

This paper presents PaSe, an extensible and inspectable DSL embedded in Haskell for expressing micro-animations. The philosophy of PaSe is to compose animations based on sequential and parallel composition of smaller animations. This differs from other animation libraries that focus more on sequential composition and have only limited forms of parallel composition. To provide similar flexibility as other animation libraries, PaSe features extensibility of operations and inspectability of animations. We present the features of PaSe with a to-do list application, discuss the PaSe implementation, and argue that the callback style of extensibility is detrimental for correctly combining PaSe features. We contrast with the GreenSock Animation Platform, a professional-grade and widely used JavaScript animation library, to illustrate this point.

==> sections/03-code.tex <==
\begin{code}
{-# LANGUAGE TemplateHaskell #-}
{-# LANGUAGE NamedFieldPuns #-}
{-# LANGUAGE MultiParamTypeClasses #-}
{-# LANGUAGE RankNTypes #-}
{-# LANGUAGE FlexibleContexts #-}
{-# LANGUAGE FlexibleInstances #-}

import Prelude hiding (seq)

import Control.Applicative (liftA2)
import Control.Monad

import Data.Functor.Const

import Lens.Micro
import Lens.Micro.TH

import Graphics.Gloss hiding (color)
import Graphics.Gloss.Interface.Pure.Game hiding (color)

main :: IO ()
main = let
  bgColor = makeColor (196 / 256) (200 / 256) (194 / 256) 1
  window = InWindow "animation-dsl" (100, 100) (100, 100)
  in do
  play window bgColor 60 () (\_ -> rectangleSolid 20 20 & Color (makeColor 1 0 0 1)) (\_ w -> w) (\_ w -> w)

str :: String
str = "str"

newtype Duration = For Float
  deriving (Ord, Eq, Show)

instance Semigroup Duration where
  (<>) = mappend

instance Monoid Duration where
  mempty = For 0
  mappend (For a) (For b) = For (a + b)

newtype Target = To Float
  deriving (Ord, Eq, Show)

data MenuWorld = MenuWorld
data GameWorld = GameWorld

x = undefined
y = undefined

menu = undefined
obscuringBox = undefined
alpha = undefined

playSound = undefined

instance (Monad m) => Functor (Animation obj m) where
  fmap = liftM

instance (Monad m) => Applicative (Animation obj m) where
  pure = return
  (<*>) = ap
\end{code}

